Scaling Down to Scale Up: A Guide to Parameter-Efficient Fine-Tuning

This paper presents a systematic overview of parameter-efficient fine-tuning methods, covering over 50 papers published between early 2019 and mid-2024. These methods aim to address the challenges of fine-tuning large language models by training only a small subset of parameters. We provide a taxonomy that covers a broad range of methods and present a detailed method comparison with a specific focus on real-life efficiency in fine-tuning multibillion-scale language models. We also conduct an extensive head-to-head experimental comparison of 15 diverse PEFT methods, evaluating their performance and efficiency on models up to 11B parameters. Our findings reveal that methods previously shown to surpass a strong LoRA baseline face difficulties in resource-constrained settings, where hyperparameter optimization is limited and the network is fine-tuned only for a few epochs. Finally, we provide a set of practical recommendations for using PEFT methods and outline potential future research directions.

==> tables/efficiency_table.tex <==
\begin{table*}[t]
% \begin{small}
\centering
\begin{tabular}{l|c|cc|c|ccc}
% \begin{tabular}{l|>{\columncolor{greenish}}c>{\columncolor{greenish}}c>{\columncolor{redish}}c|c}
\toprule
\textbf{Method} & \textbf{Type} & \textbf{Storage} & \textbf{Memory} & \textbf{Overhead} & \textbf{$<$1B} & \textbf{$<$20B} & \textbf{$>$20B} \\
\midrule
Adapters          \cite{adapters}                & \ad     & \yes & \yes & FFN        & \yes & \yes & \yes \\
AdaMix            \cite{adamix}                  & \ad     & \yes & \yes & FFN        & \yes & \no  & \no \\
SparseAdapter     \cite{sparse_adapter}          & \ad \se & \yes & \yes & FFN        & \yes & \no  & \no \\
Cross-Attn tuning \cite{cross_attention_tuning}  & \se     & \yes & \yes & \gren{no}  & \yes & \no  & \no \\
BitFit            \cite{bitfit}                  & \se     & \yes & \yes & \gren{no}  & \yes & \yes & \no \\
DiffPruning       \cite{diff_pruning}            & \se     & \yes & \no  & \gren{no}  & \yes & \no  & \no \\
Fish-Mask         \cite{fish_mask}               & \se     & \yes & \orange{maybe}\footnotemark[5] & \gren{no}  & \yes & \yes & \no \\
LT-SFT            \cite{lottery_ticket_tuning}   & \se     & \yes & \orange{maybe}\footnotemark[5] & \gren{no} & \yes & \no & \no \\
Prompt Tuning     \cite{prompt_tuning}           & \ad     & \yes & \yes & Seq.       & \yes & \yes & \yes \\
Prefix-Tuning     \cite{prefix_tuning}           & \ad     & \yes & \yes & Seq.       & \yes & \yes & \yes \\
Spot              \cite{spot}                    & \ad     & \yes & \yes & Seq.       & \yes & \yes & \no \\
IPT               \cite{ipt}                     & \ad     & \yes & \yes & FFN, seq.  & \yes & \no  & \no \\
MAM Adapter       \cite{parallel_adapter}        & \ad     & \yes & \yes & FFN, seq.  & \yes & \no  & \no \\
Parallel Adapter  \cite{parallel_adapter}        & \ad     & \yes & \yes & FFN        & \yes & \no  & \no \\
\footnotesize{Intrinsinc SAID} \cite{intrinsic_said} & \rp & \no  & \no  & \gren{no}  & \yes & \yes & \no \\
LoRa              \cite{lora}                    & \rp     & \yes & \yes & \gren{no}  & \yes & \yes & \yes \\
% DyLoRa            \cite{dylora}                  & \rp     & \yes & \yes & \no  & \gren{No}         \\
UniPELT           \cite{unipelt}                 & \ad \rp & \yes & \yes & FFN, seq.  & \yes & \no  & \no \\
\footnotesize{Compacter}   \cite{compacter}      & \ad \rp & \yes & \yes & FFN & \yes & \yes  & \no \\
\footnotesize{PHM Adapter} \cite{compacter}      & \ad \rp & \yes & \yes & FFN        & \yes & \no  & \no \\
KronA             \cite{krona}                   &     \rp & \yes & \yes & \gren{no}  & \yes & \no  & \no \\
KronA$^B_{res}$   \cite{krona}                   & \ad \rp & \yes & \yes & FFN        & \yes & \no  & \no \\
(IA)$^3$          \cite{t_few}                   & \ad     & \yes & \yes & $l_{ff}$      & \no  & \yes  & \no \\
% \footnotesize{WARP \cite{Hambardzumyan2021WARPWA}} & \ad   & \yes & \yes & \no  & Extra input                \\
% IPT               \cite{ipt}                     & \ad     & \yes & \yes & \no  & Extra input                  \\
Attention Fusion  \cite{attention_fusion}        & \ad     & \yes & \yes & Decoder    & \yes & \no  & \no \\
LeTS              \cite{lets}                    & \ad     & \yes & \yes & FFN        & \yes & \no  & \no \\
Ladder Side-Tuning \cite{ladder_side_tuning}     & \ad     & \yes & \yes & Decoder    & \yes & \yes & \no \\
FAR               \cite{far_edge}                & \se     & \yes & \orange{maybe}\footnotemark[6] & \gren{no} & \yes & \no  & \no \\
S4          \cite{design_spaces}                 &\ad \rp \se& \yes & \yes & FFN, seq.& \yes & \yes  & \no \\
\bottomrule
% Meta-Adapters     \cite{meta_adapters}           & A      & \yes & \yes & \no  & Extra FFN                  \\
% Priming           \cite{}                        & A      & \yes & \yes & \no  &                              \\
% Prompt Mapping    \cite{prompt_mapping}          & A      & \yes & \yes & \no  & Extra input                \\
% Polyhistor        \cite{polyhistor}              & A      & \yes & \yes & \no  &                              \\
% PETT              \cite{pett}                    & \rped{?}& \yes & \yes & \no  &                              \\
\end{tabular}
\vspace{2pt}
% \end{small}
\caption{Comparing \peft{} methods across storage, memory, and computational efficiency in terms of reducing backpropagation costs and inference overhead. \textbf{\ad} -- additive, \textbf{\se} -- selective, \textbf{\rp} -- reparametrization-based. Inference overhead: FFN -- extra FFN layer, seq. -- longer attention sequence, decoder -- extra transformer decoder.
% Note that S4-model has smaller inference overhead than other methods that combine Adapters and Prefix-tuning, because it uses differnt combinations of \peft{} methods on different layer (Section \rpef{sec:s4}). FishMask and FAR memory efficiency depend on weight pruning method. FishMask can significantly benefint from sparse operations hardware support (Section \rpef{sec:fishmask}).
% ^* Kronerker layer is a linear layer where weight matrix is constructed as a kroneker product of
}
\label{tab:efficiency_2}
\end{table*}


==> tables/peft_comparison_dataset_average_tall_abs_throughput.tex <==
% 
% !! Old version of the table !!
% 
% The one we are actually using is peft_comparison_dataset_average_tall.tex
% 

{
% \fontsize{9pt}{9pt}\selectfont % Custom font size
\renewcommand{\arraystretch}{0.6} % Reduces the padding within cells & making rows more compact
\begin{table}
\centering
\begin{tabular}{@{}ll|c|r|r|r|r|r@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multirow{2}{*}{Score} & \multicolumn{2}{c|}{Trainable params} & RAM & \multicolumn{2}{c}{Throughput} \\
& & & \multicolumn{1}{c|}{Millions} & \multicolumn{1}{c|}{\%} & \multicolumn{1}{c|}{\footnotesize{(GB)}} & \multicolumn{1}{c|}{Train.} & \multicolumn{1}{c}{Infer.}\\

\midrule
T5$_{Large}$ & Full tuning        & $67.22\hspace{1.8em}$ & 737.67& 100 & 20.7 & 349.6 & 12.88 \\
T5$_{Large}$ & Houlsby            & $\textbf{67.34}_{\pm9.58}$&12.69& 1.720 & 12.1 & 355.4 & 4.64 \\
T5$_{Large}$ & Pfeiffer           & $62.93_{\pm3.52}$ & 6.34   & 0.860  & 14.0 & 379.4 & 5.35 \\
T5$_{Large}$ & Parallel Adapter   & $66.78_{\pm3.85}$ & 50.41  & 6.833  & 14.7 & 430.3 & 5.42 \\
T5$_{Large}$ & IA3                & $55.06_{\pm1.80}$ & 0.34   & 0.047  & 16.2 & 435.8 & 4.21 \\
T5$_{Large}$ & Prefix tuning      & $45.05_{\pm3.89}$ & 77.31  & 10.481 & 15.4 & 395.8 & 4.59 \\
T5$_{Large}$ & Prompt tuning      & $8.97_{\pm30.91}$ & 4.42   & 0.600  & 10.6 & 380.3 & 2.45 \\
T5$_{Large}$ & LN tuning          & $64.68_{\pm4.59}$ & 0.12   & 0.017  & 14.6 & 500.4 & 6.48 \\
T5$_{Large}$ & LoRa (q and v)     & $\textbf{67.42}_{\pm2.32}$ & 2.36  & 0.320  & 14.3 & 432.5 & 6.33 \\
T5$_{Large}$ & LoRA (all)         & $\textbf{68.76}_{\pm1.83}$ & 8.65  & 1.173  & 15.9 & 282.9 & 4.84 \\
T5$_{Large}$ & KronA              & $65.68_{\pm3.27}$ & 0.22   & 0.030  & 14.6 & 381.9 & 5.13 \\
T5$_{Large}$ & MAM                & $46.90_{\pm6.47}$ & 171.07 & 23.191 & 16.6 & 370.8 & 3.16 \\
T5$_{Large}$ & Compacter          & $64.48_{\pm1.81}$ & 0.30   & 0.041  & 14.4 & 284.1 & 3.37 \\
T5$_{Large}$ & Compacter++        & $64.78_{\pm2.23}$ & 0.15   & 0.021  & 13.9 & 333.6 & 4.06 \\
T5$_{Large}$ & Unipelt            & $44.10_{\pm15.48}$& 86.22  & 11.689 & 16.7 & 213.5 & 3.59 \\
\addlinespace
T5$_{3B}$    & Full tuning        & $74.83\hspace{1.8em}$& 2851.60 & 100 & 32.9 & 346.9 & 1.36 \\
T5$_{3B}$    & Houlsby            & $74.66_{\pm1.68}$ & 12.69 & 0.445 &  9.3 & 323.1 & 0.69 \\
T5$_{3B}$    & Pfeiffer           & $69.92_{\pm5.61}$ & 6.34  & 0.223 &  9.6 & 357.1 & 0.75 \\
T5$_{3B}$    & Parallel Adapter   & $74.15_{\pm0.88}$ & 50.41 & 1.768 & 10.0 & 356.4 & 0.75 \\
T5$_{3B}$    & IA3                & $41.77_{\pm0.50}$ & 1.38  & 0.048 & 10.8 & 360.4 & 0.45 \\
T5$_{3B}$    & Prefix tuning      & $48.90_{\pm5.37}$ & 77.25 & 2.709 & 12.3 & 365.1 & 0.56 \\
T5$_{3B}$    & Prompt tuning      & $8.38_{\pm0.50}$  & 17.69 & 0.621 &  8.9 & 346.7 & 0.36 \\
T5$_{3B}$    & LN tuning          & $72.95_{\pm1.38}$ & 0.12  & 0.004 &  9.7 & 488.2 & 0.88 \\
T5$_{3B}$    & LoRa (q and v)     & $\textbf{75.49}_{\pm1.71}$& 3.93  & 0.138 & 9.6 & 357.4 & 0.91 \\
T5$_{3B}$    & LoRA (all)         & $\textbf{75.22}_{\pm1.28}$& 25.17 & 0.883 & 10.6 & 243.7 & 0.74 \\
T5$_{3B}$    & KronA              & $71.98_{\pm0.57}$ & 0.41  & 0.014 & 10.8 & 286.3 & 0.68 \\
T5$_{3B}$    & MAM                & $45.57_{\pm4.67}$ & 171.07& 5.999 & 14.2 & 293.2 & 0.49 \\
T5$_{3B}$    & Compacter          & $70.72_{\pm0.87}$ & 0.30  & 0.011 & 9.7 & 248.1 & 0.36 \\
T5$_{3B}$    & Compacter++        & $71.00_{\pm1.62}$ & 0.15  & 0.005 & 9.5 & 301.6 & 0.45 \\
T5$_{3B}$    & Unipelt            & $47.16_{\pm4.84}$ & 316.70& 11.106& 12.8 & 176.8 & 0.37 \\
\addlinespace
% \midrule
T5$_{11B}$   & Full tuning        & $73.25\hspace{1.8em}$ & 11307.32 & 100  \\
T5$_{11B}$   & Houlsby            & $\textbf{76.16}_{\pm1.47}$  & 12.69 & 0.112 & 28.8 & 293.5 & 0.24     \\
T5$_{11B}$   & Pfeiffer           & $50.72_{\pm1.69}$  & 6.34 & 0.056 & 28.6 & 327.2 & 0.22      \\
T5$_{11B}$   & Parallel Adapter   & $68.74_{\pm12.73}$ & 50.41 & 0.446 & 29.0 & 318.6 & 0.20     \\
T5$_{11B}$   & IA3                & $61.05_{\pm3.42}$  & 3.48 & 0.031 & 31.0 & 317.1 & 0.15      \\
T5$_{11B}$   & Prefix tuning      & $51.93_{\pm2.21}$  & 1211.99 & 10.719 & 35.6 & 62.5 & 0.12  \\
T5$_{11B}$   & Prompt tuning      & -                  & 70.78 & 0.626 & 30.2 & 286.2 & 0.12     \\
T5$_{11B}$   & LN tuning          & $\textbf{73.77}_{\pm0.93}$  & 0.12 & 0.001 & 28.4 & 376.8 & 0.32      \\
T5$_{11B}$   & LoRa (q and v)     & $\textbf{76.20}_{\pm1.27}$  & 20.05 & 0.177 & 28.9 & 296.2 & 0.31     \\
T5$_{11B}$   & LoRA (all)         & $\textbf{76.58}_{\pm2.16}$  & 91.23 & 0.807 & 30.8 & 207.2 & 0.26     \\
T5$_{11B}$   & KronA              & $72.13_{\pm7.30}$  & 0.77 & 0.007 & 33.2 & 237.6 & 0.23      \\
T5$_{11B}$   & MAM                & $51.49_{\pm0.54}$  & 1262.39 & 11.164 &   &   &    \\
T5$_{11B}$   & Compacter          & $\textbf{74.33}_{\pm1.40}$  & 0.30 & 0.003 & 28.6 & 222.2 & 0.12      \\
T5$_{11B}$   & Compacter++        & $\textbf{74.72}_{\pm0.82}$  & 0.15 & 0.001 & 28.5 & 285.2 & 0.14      \\
T5$_{11B}$   & Unipelt            & $52.29_{\pm3.09}$  & 1224.78 & 10.832 & 36.4 & 56.5 & 0.08   \\
\bottomrule
\end{tabular}
\caption{Average model performance on our collection of datasets (Section \ref{sec:comparison_datasets}). Standard deviation is computed over datasets. Raw results (about \red{600} experiments) are available in Appendix \ref{sec:peft_comparison_raw}. \textbf{Bold} values outperform full fine-tuning.
}
\label{tab:peft_comparison_tall}
\end{table}
}

==> tables/scale_table.tex <==
\newcommand{\unsim}{\mathord{\sim}}

% NOTE: For IPT, we train 56% of parameters, but then we throw away the autoencoder encoder, so in some sence, only 42% are chaged

\begin{table*}[ht]
\centering
\begin{small}
\begin{tabular}{l|cc|ccc}
% \begin{tabular}{l|>{\columncolor{greenish}}c>{\columncolor{greenish}}c>{\columncolor{redish}}c|c}
\toprule
% \textbf{Method}                                     & Trainable parameters & \textbf{<1B} & \textbf{<20B} & \textbf{>20B} \\
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{2cm}{\centering\textbf{\%Trainable parameters}} & \multirow{2}{2cm}{\centering\textbf{\%Changed parameters}} & \multicolumn{3}{c}{\textbf{Evaluated on}} \\
& & & \textbf{\textless1B} & \textbf{\textless20B} & \textbf{\textgreater20B} \\
\midrule
Adapters          \cite{adapters}                   & 0.1 - 6    & 0.1 - 6      & \yes & \yes & \yes \\
AdaMix            \cite{adamix}                     & 0.1 - 0.2  &0.1 - 0.2     & \yes & \no  & \no  \\
SparseAdapter     \cite{sparse_adapter}             & 2.0        & 2.0          & \yes & \no  & \no  \\
BitFit            \cite{bitfit}                     & 0.05 - 0.1 &0.05 - 0.1    & \yes & \yes & \yes \\
DiffPruning       \cite{diff_pruning}               & 200        & \textbf{0.5} & \yes & \no  & \no  \\
Fish-Mask         \cite{fish_mask}                  & 0.01 - 0.5 &0.01 - 0.5    & \yes & \yes & \no  \\
Prompt Tuning     \cite{prompt_tuning}              & 0.1        & 0.1          & \yes & \yes & \yes \\
Prefix-Tuning     \cite{prefix_tuning}              & 0.1 - 4.0  & 0.1 - 4.0    & \yes & \yes & \yes \\
IPT               \cite{ipt}                        & 56.0       & 56.0     & \yes & \no  & \no \\
MAM Adapter       \cite{parallel_adapter}           & 0.5        & 0.5          & \yes & \no  & \no  \\
Parallel Adapter  \cite{parallel_adapter}           & 0.5        & 0.5          & \yes & \no  & \no  \\
Intrinsinc SAID   \cite{intrinsic_said}             & 0.001 - 0.1& \textbf{100}          & \yes & \yes & \no  \\
LoRa              \cite{lora}                       & 0.01 - 0.5 & \textbf{$\unsim$30}   & \yes & \yes & \yes \\
UniPELT           \cite{unipelt}                    & 1.0        & 1.0      & \yes & \no  & \no  \\ 
Compacter         \cite{compacter}                  & 0.05-0.07  & \textbf{$\unsim$0.1} & \yes & \yes & \no  \\
PHM Adapter       \cite{compacter}                  & 0.2        & \textbf{$\unsim$1.0} & \yes & \no  & \no  \\
KronA             \cite{krona}                      & 0.07       & \textbf{$\unsim$30.0}& \yes& \no  & \no  \\
KronA$^B_{res}$   \cite{krona}                      & 0.07       & \textbf{$\unsim$1.0} & \yes & \no  & \no  \\
(IA)$^3$          \cite{t_few}                      & 0.02       & 0.02     & \no  & \yes & \no  \\
% IPT               \cite{ipt}                        &            &          & \yes &      &      \\
Ladder Side-Tuning\cite{ladder_side_tuning}         & 7.5        & 7.5      & \yes & \yes & \no  \\
FAR               \cite{far_edge}                   & 6.6-26.4   & 6.6-26.4 & \yes & \no  & \no  \\
S4-model          \cite{design_spaces}              & 0.5        &\textbf{\textgreater 0.5} & \yes & \yes & \no  \\

% WARP              \cite{Hambardzumyan2021WARPWA}    &            & \yes &      &      \\
% LeTS              \cite{}                           & \yes &      &      \\
% Cross-Attn tuning \cite{cross_attention_tuning}     & \yes &      &      \\
% Attention Fusion  \cite{attention_fusion}           & \yes &      &      \\
% LT-SFT            \cite{}                           & \yes &      &      \\
% Priming           \cite{}                           & \yes &      &      \\
% Polyhistor        \cite{polyhistor}                 & \yes &      &      \\
% PETT              \cite{pett}                       & \yes &      &      \\
\bottomrule
\end{tabular}
\vspace{2pt}
\end{small}
\caption{What model sizes \peft{} methods have been evaluated on and their typical amount of trainable parameters.}
\label{tab:scale_table}
\end{table*}

